Optimal Dynamic Distributed MIS

Finding a maximal independent set (MIS) in a graph is a cornerstone task in distributed computing. The local nature of an MIS allows for fast solutions in a static distributed setting, which are logarithmic in the number of nodes or in their degrees. The result trivially applies for the dynamic distributed model, in which edges or nodes may be inserted or deleted. In this paper, we take a different approach which exploits locality to the extreme, and show how to update an MIS in a dynamic distributed setting, either \emph{synchronous} or \emph{asynchronous}, with only \emph{a single adjustment} and in a single round, in expectation. These strong guarantees hold for the \emph{complete fully dynamic} setting: Insertions and deletions, of edges as well as nodes, gracefully and abruptly. This strongly separates the static and dynamic distributed models, as super-constant lower bounds exist for computing an MIS in the former. Our results are obtained by a novel analysis of the surprisingly simple solution of carefully simulating the greedy \emph{sequential} MIS algorithm with a random ordering of the nodes. As such, our algorithm has a direct application as a $3$-approximation algorithm for correlation clustering. This adds to the important toolbox of distributed graph decompositions, which are widely used as crucial building blocks in distributed computing. Finally, our algorithm enjoys a useful \emph{history-independence} property, meaning the output is independent of the history of topology changes that constructed that graph. This means the output cannot be chosen, or even biased, by the adversary in case its goal is to prevent us from optimizing some objective function.

==> correlation.tex <==
%\subsection{Correlation Clustering}
\ktodo{should this also be moved into the intro? we are not saying much here, will have to say only that the cluster center is the mis node...}
Consider the following clustering (i.e.\ partitioning of the graph vertices) obtained from any MIS and an ordering $\pi$ over the nodes. Every node in $\M$ represents a cluster which is denoted by its ID. A node that is not in $\M$ is belongs to the cluster corresponding to its neighbor in $\M$ of the lowest order according to $\pi$. Since $\M$ is maximal, the above is indeed a partition of the entire node set.

Since in our MIS algorithm each node knows the random IDs of its neighbors and their states, it can easily deduce the ID of the cluster to which it belongs.
One can easily verify that the clustering induced by the above definition from the MIS that is obtained by our algorithm is exactly the same clustering that is produced by Algorithm \emph{KwikCluster} in~\cite{AilonCN08}. It follows that the clustering obtained from our protocol yields an expected $3$-approximation to the optimal correlation clustering, as proved in Theorem 11 of~\cite{AilonCN08}.

%It remains to analyze the required modifications to the MIS protocol in order for the nodes to be able to output not only whether they are in $\M$, but in the case of not being in $\M$, the identity of their neighbor in $\M$ of minimal order. It is an easy exercise to show that the following two changes yield a working protocol: (1) if a node changes its state to $\M$, it outputs its random number (of $O(\log(n))$ bits) that determines it's place in the random ordering, and (2) every node maintains in its internal memory the list of random numbers associated with all of it's neighbors in $\M$. The properties of the protocol are maintained, where the messages are limited to $O(\log(n))$ bits and the internal memory remains bounded by $O(\Delta \log(n))$.


